Gabriel's theorem and birational geometry

Extending work of Meinhardt and Partsch, we prove that two varieties are isomorphic in codimension c if and only if certain quotients of their categories of coherent sheaves are equivalent. This result interpolates between Gabriel's reconstruction theorem and the fact that two varieties are birational if and only if they have the same function field.

==> bir.tex <==
%!TEX root = MASTER.tex
\section{Birational skeleton}
%Before we complete the proof, we introduce the notion of birational skeleton of $X$.
%This is a locally ringed space $^cX$ which remembers the birational geometry in codimension $c$ of $X$.
%\begin{defn}
%	Define $^cX$ to be the locally ringed space as...
%\end{defn}
%\begin{prop}
%	Let $X$ and $Y$ be...
%	Then $X$ and $Y$ are isomorphic in codimnesion $c$ if and only if $^cX$ and $^cY$ are isomorphic as locally ringed spaces.
%\end{prop}
%
%
%Vabb\`o, forse questo non \`e l'approccio giusto.
%Bisognerebbe forse andare dirattamente su $\K(X)$ e il reticolo degli anelli locali. Boh, bisogna capire un po' meglio la situazione.
%
%
%
%
%In ogni caso ci vuole un risultato in questa sezione che dice che se tot \`e vero allora X e Y sono isomorfi in codimensione c.
%E poi nella prossima sezione mettiamo tutto insieme e diciamo che se le categorie sono equivalenti allora tot, e dunque sono isomorfi in codimensione c.

As we are working with irreducible schemes, we can reindex our quotient categories by codimension, by $\cat C_{i}=\cat C^{n-i-1}$.

\begin{defn}
We define the topological space $^cX$ as follows. Consider the set 
\begin{align*}
	\bigcup_{d \leq c}\lbrace P \in \cat C^{d}(X) \mid P \mbox{ is minimal}\rbrace
\end{align*}
The closure $\bar{P}$ of a point $P$ coming from $\cat C^{d}(X)$ is defined by $\bar{P}=\cup_{d < j \leq c}\lbrace Q \in \cat C^{ j}(X) \mid Q \in S(P) \rbrace$.
These subsets form a basis of closed subsets for $^cX$.
\end{defn}

\todo{da riscrivere con le referenze giuste} Propositions \ref{min1}, \ref{min2} give us an injection $^cX \xrightarrow{i} |X|$.
It is immediate to verify that $i$ induces a bijection between $^cX$ and the subspace of $|X|$ given by points of codimension at most $c$.

The following is immediate.
\begin{prop}
An equivalence $\cat C^{ c}(Y) \simeq \cat C^{ c}(X)$ induces a homeomorphism $^cX \xrightarrow{\phi} {^cY}$.
\end{prop}

\todo{opzione 1(fancy)}

We give $^cX$ a structure of ringed space in the following way. Let $S_U$ be the serre subcategory of $C^{c}$ generated by the elements $P \mid P \notin U$. Then we define $\O_{^cX}(U)=\hom_{\cat C^c/S_U}(\O_X,\O_X)$. Clearly the isomorphism $^cX \xrightarrow{\phi} ^cY$ in the previous proposition extends to this structure.

\begin{rmk}
A map $F \rightarrow G$ in $\cat C^c/S_U$ can be represented as a roof $F \xleftarrow{s} E \xrightarrow{s'} G$ where $\ker s, \coker s, \coker s'$ are supported on the complement of $U$.
\end{rmk}

\begin{lem}
We have 
$$\Hom_{\cat C^c/S_U}(F,G)= \varinjlim_{U \subseteq W} \Hom_{\Coh(W)}(F_W,G_W)$$
where $W$ runs over Zariski open subsets of $X$.
\end{lem}
\begin{proof}
We will define mutually inverse maps $\hom_{\cat C^c/S_U}(F,G)\leftrightarrow \lim_{U \subseteq W}\hom_{\Coh(W)}(F_W,G_W)$, following \cite[3.6]{MP}.

Let $W$ be an open subset containing $U$, and $f:F \rightarrow G$ a morphism. Consider a coherent sheaf $E$ such that $E_W = \Gamma_f \subset F \oplus G$. Then the roof $F \xleftarrow{\mathrm{pr}_1} E \xrightarrow{\mathrm{pr}_2} G$ represents an element $f \in \hom_{\cat C^c/S_U}(F,G)$. One can check that this element is unique exactly as in \emph{loc.cit.}

Consider now a roof $F \xleftarrow{s} E \xrightarrow{s'} G$. Let $W$ be the complement of $\mathrm{supp}(\ker(s)) \cup \mathrm{supp}(\coker(s))$. We associate to it the map $s^{-1}\cdot s':F \rightarrow G$. Again we can check that this element is well defined and that the two maps are inverse to each other as in \emph{loc. cit.}
\end{proof}
\todo{bisogna scrivere una dimostrazione completa}

%\begin{lem}
%We have $$\O_{^cX}(U) \simeq \lim_{U \subseteq W} \hom_{\Coh(W)}(\O_W, \O_W)$$ where $W$ runs over Zariski open subsets of $X$.
%\end{lem}

\begin{cor}
Consider the locally ringed space $(^cX,\O_X)$ obtained by restricting the canonical sheaf and Zariski topology to the subset $^cX$. Then we have $$(^cX,\O_X) \simeq (^cX, \O_{^cX}).$$
\end{cor}
\begin{proof}
We have 
	$$ \O_{^cX}(U)=\hom_{\cat C^c/S_U}(\O_X,\O_X)= \varinjlim_{U \subseteq W} \hom_{\Coh(W)}(\O_W, \O_W) $$
	and additionally $\hom_{\Coh(W)}(\O_W, \O_W)=\O_W(W)$ which allows us to conclude immediately.

\end{proof}

\begin{lem}\label{lociso}
Let $R, R'$ be finitely generated and integral $A$-algebras and let $p\subset R,p' \subset R'$ be prime ideals. Suppose there is an isomorphism of $A$-algebras $R_p \simeq R'_{p'}$. Then there are open subschemes $U \subset \Spec(R), U' \subset \Spec(R')$ containing $p$ and $p'$ respectively such that $U \simeq U'$ as $\Spec(A)$-schemes.
\end{lem}
\begin{proof}
Consider the composition $R' \rightarrow R'_{p'} \rightarrow R_p$. Consider a finite set of generators $x_1, \ldots, x_n$ for $R$ as an $A$-algebra. Their images will be in the form $r_1/s_1, \ldots , r_n/s_n$ where $r_1,\ldots,r_n$ belong to $R$ and $s_1,\ldots,s_n$ belong to $R \setminus p$. This shows that the image of $R'$ is contained in $S^{-1}R$ where $S=\lbrace s_1^{i_1} \ldots s_n^{i_n}\rbrace$. The inclusion $\Spec(S^{-1}R)\subset \Spec(R)$ is open and it contains the point $p$. This shows that we have a map $W \rightarrow \Spec(R')$ where $W$ is a neighbourhood of $p$, and the map send $p$ to $p'$. By restricting to open subsets $U$ of $\Spec(R)$ and $U'$ of $\Spec(R')$ containing $p$ and $p'$ we may further assume that the map is unramified, quasi-finite and of degree one at all points, i.e. an isomorphism.
\end{proof}

\begin{lem}
Suppose we have an isomorphism of locally ringed spaces $^cX \xrightarrow{\phi} {^cY}$.
Then $X \sim^c Y$ and the morphism inducing the equivalence agrees with $\phi$ on $^cX$.
\end{lem}
\begin{proof}
Given a point $p \in ^cX$ isomorphism of local rings $\O_{Y,\phi(p)}\simeq \O_{X,p}$ induces an isomorphism $U \simeq V$ of Zariski neighborhoods of $p, \phi(p)$, sending $p$ to $\phi(p)$. Moreover $X$ and $Y$ are reduced and separated so any two of these isomorphisms must agree on the intersection of the respective open neighborhoods. A simple gluing argument completes the proof.
\end{proof}

\todo{controllare, scrivere meglio}

\begin{cor}
Suppose we have an isomorphism $\psi: \cat C^{ c}(Y) \rightarrow \cat C^{ c}(X)$.
Then $X$ and $Y$ are isomorphic in codimension $c$ and the isomorphism is compatible with the isomorphism $\psi: ^cX \rightarrow ^cY$ of locally ringed spaces.
\end{cor}
\begin{proof}

\end{proof}

\todo{dovremmo specificare che l'isomorfismo in codimensione c non induce necessariamente la mappa sulle categorie abeliane. Sarebbe ganzo avere un esempio in cui queste categorie si possono calcolare esplicitamente.}

%\todo[inline]{opzione 2(semplice)}
%
%Our aim is to construct a corresponding isomorphism $U^c_X \xrightarrow{\phi} U^c_Y$, where $U^c_X, U^c_Y$ are open subschemes containing all points of codimension $\leq c$. The next lemma shows that it is sufficient to prove that all the local rings are isomorphic.
%
%\begin{lem}\label{lemmastupido}
%Assume that for every closed point $p \in {^cX}$ there is a local ring isomorphism $\O_{Y,\phi(p)}\simeq \O_{X,p}$, and moreover that all these isomorphisms agree when restricted to $\K(X) \simeq \K(Y)$.
%Then $X \sim^c Y$ and the morphism inducing the equivalence agrees with $\phi$ on the closed points of $^cX$.
%\end{lem}
%\begin{proof}
%The isomorphism of local rings $\O_{Y,\phi(p)}\simeq \O_{X,p}$ induces an isomorphism $U \simeq V$ of neighborhoods of $p, \phi(p)$, sending $p$ to $\phi(p)$. Moreover $X$ and $Y$ are reduced and separated so two of these isomorphsims must agree on the intersection of the respective open neighborhoods. A simple gluing argument completes the proof.
%\end{proof}
%
%We already know that an isomorphism in codimension $0$ exists. We will inductively produce an isomorphism in codimension $d$ for all $d \leq c$. In the following we will assume given an isomorphism $\psi: \cat C^{ c}(Y) \rightarrow \cat C^{ c}(X)$.
%
%\begin{prop}
%$X \sim^1 Y$ and the map is compatible with the topological map $\psi$ on $^1X$.
%\end{prop}
%\begin{proof}
%Fix an irreducible divisor $D$ of $X$.
%Consider the Serre subcategory $S_{\neq D}$ of $\cat C^{ 1}(X)$ defined as the minimal Serre subcategory containing all the minimal objects of $\cat C^{ 1}(X)$ whose support is not $D$.
%Define $C_D=\cat C^{ 1}(X)/S_{\neq D}$.
%Then $$ \hom_{C_D}(\O_X,\O_X)=\lim_{D \in U}(\hom_{\Coh(X)}(\O_U,\O_U))=\O_{X,D}.$$
%This construction passes through the isomorphism $\psi$ so it gives us the isomorphism of local rings we need to apply lemma \ref{lemmastupido}, which allows us to conclude.
%\end{proof}
%
%\begin{prop}
%Suppose $d \geq 2$, and suppose that $X \sim^{d-1} Y$ and that the map is compatible with the map $\psi$ on $^{d-1}X$.
%Then $X \sim^{d} Y$ and the map is compatible with $\psi$ on $^dX$.
%\end{prop}
%\begin{proof}
%Let $U_X\simeq U_Y$ be an isomorphsim in codimension $d-1$ compatible with $\psi$ on $^{d-1}X$. let $p \in X$ be a point of codimension $d$.
%We may assume without loss of generality that $p \notin U_X$. We say that an open subset $U'_X \subseteq U$ has property $(*,p)$ iff $(U' \cup p) \cap ^cX$ is open in $^dX$.
%This is equivalent to asking that $U'$ is the intersection of a neighborhood of $p$ and $U_X$.
%Then it's easy to see that $\cap_{U' \mid *} U' = \Spec(\O_{X,p}) \setminus p$.
%This property only depends on the intersection with $^{d-1}X$ so the image of an open subscheme of $X$ satisfying $(*,p)$ is an open subset of $Y$ satisfying $(*, \phi(p))$ and vice versa.
%Then the intersections of all such open subschemes must be isomorphic, so we have an isomorphism $$\Spec(\O_{X,p}) \setminus p \simeq \Spec(\O_{Y,\phi(p)}) \setminus \phi(p).$$
%
%Now we use the following fact: given a normal Noetherian scheme $S$ and a closed subset $V$ of codimension $2$ or more the restriction $\O_S(S) \rightarrow \O_S(S\setminus V)$ is an isomorphism.
%Then the isomorphism $\Spec(\O_{X,p}) \setminus p \simeq \Spec(\O_{Y,\phi(p)}) \setminus \phi(p)$ induces an isomorphism on global sections, which in turn is the isomorphism $\O_{X,p} \simeq \O_{Y,\phi(p)}$ we are looking for.
%\end{proof}
%
%\begin{cor}
%Suppose we have an isomorphism $\psi: \cat C^{ c}(Y) \rightarrow \cat C^{ c}(X)$.
%Then $X$ and $Y$ are isomorphic in codimension $c$ and the isomorphism is compatible with the map $\psi: ^cX \rightarrow ^cY$.
%\end{cor}


%\section{Proof}
%Here we put the two previous sections together and prove our main result.
%Suppose we have a $\k$-linear equivalence $\Phi_k \colon \cat C_k(X) \simeq \cat C_k(Y)$.
%Since an equivalence will take minimal objects to minimal objects, $\Phi$ will induce equivalences $\Phi_h\colon \cat C_h(X) \to \cat C_h(Y)$ for all $h \geq k$.
%In particular, via Proposition \ref{ff}, we have an equivalence between $\K(X) \simeq \K(Y)$.
%From this it follows that we have an isomorphism $\K(X) \simeq \K(Y)$.
%
%How do we prove now that the lattice of subrings given by all local rings are preserved?


==> non.tex <==
%!TEX root = MASTER.tex
\section{Noncommutative}

\subsection*{Non-commutative birational invariants?}
\begin{prop}
	Let $R$ be a graded $\k$-algebra satisfying some assumptions (like the ones for the graded Goldie theorem).
	Then at some point the function field shows up.
\end{prop}
\begin{proof}
	L'idea mi sembra abbastanza evidente, ma non riesco a renderla precisa.
	Chiama $\cat B$ il quoziente e chiama $F$ il campo delle funzioni.
	A ogni elemento $s^{-1}a \in F$, con $\deg s = d = \deg a$, associo la mappa nel quoziente
	\begin{align*}
		R \stackrel {\cdot s} \leftarrow R(-d) \stackrel {\cdot a} \to R
	\end{align*}
	Modulo non aver confuso destra e sinistra, questo d\`a un morfismo $F \to \End_{\cat B}(R)$.
	Ma non so ancora come costruire l'inverso.
\end{proof}

\subsection{Example?}

Let $R$ be a graded ring.
Assume $R$ is both non-negatively graded and noetherian.
I don't think it matters if it's generated in degree one or not.
Let $\grmod(R)$ be the category of finitely generated graded $R$-modules.
Let $\cat T$ be the subcategory of torsion modules.
When $R$ is finite type over a field $\k$, this coincides with the subcategory of modules which are finite dimensional as $\k$-vector spaces.
Notice that $\cat T$ coincides with the smallest Serre subcategory containing all minimal objects.

The quotient $\cat A = \grmod(R)/\cat T$, sometimes called the \emph{tails category}, is viewed as the category of coherent sheaves on a non-commutative proj scheme, which we denote by $X = \Proj R$.
This interpretation is due to what known as Serre's theorem, which says that when $R$ is commutative there is indeed an equivalence $\grmod(R)/\cat T = \Coh(\Proj(R))$.

\begin{prop}
	The dimension of $\cat A$ as defined earlier coincides with the Krull dimension of $R$ as a graded ring.
\end{prop}
\john{boh, secondo me \`e vero}

Suppose now $R$ is a ring where all non-zero homogeneous elements satisfy the Ore conditions. \todo{or whatever the fuck it needs to satisfy}
One may then form its field of fractions $F$, consisting of quotients $a/b$ where $a,b$ are both homogeneous.
Inside $F$, there is $F_0 \subset F$, consisting of elements $a/b$ where $\deg a = \deg b$.
This field $F_0$ is interpreted as being the function field $\K(X)$ of our non-commutative scheme $X$.

\begin{prop}\label{nonso}
	Let $\cat B$ be the penultimate quotient.
	Then $\cat B = \mod(F_0)$.
\end{prop}
In particular, two non-commutative projective schemes which are isomorphic in some codimension (in our categorical sense) will be birational in the sense that they have Morita equivalent function fields.
For example, \cite{presotto} provides many interesting examples of non-isomorphic but birational non-commutative surfaces.
\begin{proof}
	It's probably easy to see that any module becomes isomorphic to $R^{\oplus n}$ for some $n$, since everything has a presentation.
	
	What's a morphism $R \qto R$ in the quotient?
	Well, it's a roof $R \ot Q \to R$ where $Q \to R$ has kernel and cokernel being something.
	This something is basically anything which is not a free module.
	How do we get the function field?
	Well, let $a,b$ be two homogeneous elements of degree $d$.
	Consider $R(-d) \to R$ given by multiplication by $b$, and $R(-d) \to R$ given by multiplication by $a$.
	Then $R \ot R(-d) \to R$ corresponds to the element $a/b$ in the function field.
	In other words, $\End_{\text{quotient}}(R,R) = F_0$.
\end{proof}

\subsubsection{Noncommutative flop}
It would be amazing if we could conclude this paper with an example of two algebras which weren't isomorphic as non-commutative spaces, but were isomorphic in some codimension (and not just birational).

Unfortunately, the example of Atiyah does not look like it could be made non-commutative easily.
He takes $\k[x,y,z,w]$ and looks at the singular quadric threefold $X$, given by equation $xy - zw = 0$.
Blowing up the singular point, you get a smooth guy $W$.
The exceptional locus of $W \to X$ is $\P^1\times \P^1$.
Contracting the two projective lines you get two threefolds $Y^+$, $Y^-$ which are resolutions of $X$.
This shows in dimension three there aren't always ``minimal resolutions''.
I think in this case $Y^+$ and $Y^-$ are actually isomorphic, but the induced birational map $Y^+ \to X \ot Y^-$ is the famous flop (it does not extend to a regular map).

One would like to make this non-commutative, but I wouldn't know how.
Here's one thing we may notice.
Let $A$ be the coordinate ring of $X$.
Since $Y^\pm$ is projective over $X$, it may be described by a graded $A$-algebra.
Obviously this algebra is not generated in degree one.
One could try to make this non-commutative by declaring that some elements in degree one commute up to a root of unity, like $st = qts$ for some $q$.
This would roughly mean making the $\P^1$ non-commutative.
But apparently there aren't any non-commutative $\P^1$'s.
So maybe the thing to do is have a higher dimensional flop, where we deform the contracted $\P^2$.

Or maybe even the following.
Blow up a point in affine 3-space, the exceptional locus is a $\P^2$.
Deform the $\P^2$ to two different birational $\P^2$s in the sense of Presotto.
Does this give what we want?

